BIMC: The Bayesian Inverse Monte Carlo method for goal-oriented uncertainty quantification. Part II

In Part I (arXiv:1911.00619) of this article, we proposed an importance sampling algorithm to compute rare-event probabilities in forward uncertainty quantification problems. The algorithm, which we termed the "Bayesian Inverse Monte Carlo (BIMC) method", was shown to be optimal for problems in which the input-output operator is nearly linear. But applying the original BIMC to highly nonlinear systems can lead to several different failure modes. In this paper, we modify the BIMC method to extend its applicability to a wider class of systems. The modified algorithm, which we call "Adaptive-BIMC (A-BIMC)", has two stages. In the first stage, we solve a sequence of optimization problems to roughly identify those regions of parameter space which trigger the rare-event. In the second stage, we use the stage one results to construct a mixture of Gaussians that can be then used in an importance sampling algorithm to estimate rare event probability. We propose using a local surrogate that minimizes costly forward solves. The effectiveness of A-BIMC is demonstrated via several synthetic examples. Yet again, the modified algorithm is prone to failure. We systematically identify conditions under which it fails to lead to an effective importance sampling distribution.

==> makefile <==
papername=ms
suppname=part_2_supplement


TEX = latexmk -f -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make- -bibtex 

.PHONY: clean paper supplement

all: paper supplement

paper: 
	${TEX} ${papername}

supplement:
	${TEX} ${suppname}

bib: paper supplement
	bibtex ${papername}
	bibtex ${suppname}

clean:
	rm -f *.aux *.log *.dvi *.blg *.bbl \
          *.fls *.fdb_latexmk *.out *.spl    \
          *.brf *.snm *.toc *.nav       \
		  *.pdfsync *.pdf 
	@echo Cleaned ....! 



==> part_2_files/dimension_reduction.tex <==
\section{Dimension Reduction}
\label{section:dim_red}

\subsection{Motivation}

To illustrate the possibility of dimension reduction, we again analyze the
affine-Gaussian case. For ease of exposition, we assume that the nominal
distribution $p(\uq)$ is a standard normal, $\mathcal{N}\left(\boldsymbol{0},
{I}\right)$. We don't lose any generality in this case, as this can be
accomplished via a simple change of coordinates.

Let $f(\uq) = \vect{v}^T\uq + \beta$ and 
$p(\uq) = \mathcal{N}(\boldsymbol{0}, {I})$, for some $\vect{v}
\in \mathbb{R}^m$ and $\beta \in \mathbb{R}$. Denote by $\hat{\vect{v}}
= \vect{v} / \|\vect{v}\|$. Now, select $\hat{{V}}$ so that it's
columns form an orthonormal basis for 
$\mathbb{R}^m \textbackslash \,\text{span}(\hat{\vect{v}})$. Then, we have, for
any $\uq$:

\begin{align}
    \begin{split}
        \uq &= \hat{\vect{v}}\hat{\vect{v}}^T \uq + 
            \hat{{V}}\hat{{V}}^T\uq\\
            &= \hat{\boldsymbol{v}} x_r + \hat{{V}}\uq_{\perp}\\
    \end{split}
\end{align}

where $x_r := \hat{\boldsymbol{v}}^T\uq$ and 
$\uq_{\perp} := \hat{{V}}^T\uq$.

Using this decomposition of the parameter space, notice that 

\begin{align*}
    f(\uq) &= \vect{v}^T \uq + \beta\\
           &= \|\vect{v}\| x_r + \beta\\
           &= f(x_r),
\end{align*}

and, 

\begin{align}
    \label{eq:prior_decomp}
    p(\uq) &= p_r(x_r) p_{\perp}(\uq_{\perp}), 
\end{align}

where, $p_r(x_r) = \mathcal{N}\left(0, 1\right)$ and
$p_{\perp} = \mathcal{N}\left(\boldsymbol{0}_{\perp},
{I}_{\perp}\right)$. Hence, such a decomposition of the parameter space
enables one to express ideal IS density, $q^*$, as 

\begin{align}
    \label{eq:ideal_is_decomp}
    \begin{split}
    q^*(\uq) &= \ind_{\DT}(f(\uq))p(\uq)\\
             &= \ind_{\DT}(f(x_r))p_r(x_r)p_{\perp}(\uq_{\perp})\\
             &= q^*_r(x_r)p_{\perp}(\uq_{\perp})
    \end{split}
\end{align}

Note that these relations are exact, no approximations have been made yet. 
This suggests that $q^*$ differs from $p(\uq)$ only in the subspace
$\text{Range}(\hat{\vect{v}}\hat{\vect{v}}^T)$. This difference is captured in
$q^*(x_r)$. 

The rare event probability calculation becomes:

\begin{align}
    \begin{split}
    \mu &= \int_{\mathbb{R}^m} \ind_{\DT}(f(\uq))p(\uq)\mathrm{d}\uq\\
        &= \int \ind_{\DT}(f(x_r))p(x_r)p(\uq_{\perp})\mathrm{d}x_r
            \mathrm{d}\uq_{\perp}\\
        &= \int\ind_{\DT}(f(x_r))p(x_r)\mathrm{d}x_r
    \end{split}
\end{align}

This means that the rare event probability can be computed entirely in the
1-dimensional subspace, $\text{Range}(\hat{\vect{v}}\hat{\vect{v}}^T)$.
Hence, now the problem is to approximate $q^*_r(x_r)$ with 
an appropriate importance sampling density, say $q_r(x_r)$. 
Since this task is to be performed in
only one dimension, it is much easier than working in the full $m$-dimensional 
space. 

In this section, we showed that the ideal IS density is nothing but $p(\uq)$ in
directions where $f(\uq)$ is flat, and that dimension reduction can be achieved
if these directions are marginalized (integrated) away. To generalize the idea
of dimension reduction to nonlinear $f$ and arbitrary $p(\uq)$, we start by
making the following observations about the affine-Gaussian case. The
decomposition of $q^*$ as in the \cref{eq:ideal_is_decomp} is enabled by:

\begin{itemize}
    \item The knowledge of directions where $f(\uq)$ appears flat and where it's
        varying.
    \item The decorrelation of these two subspaces with respect to the prior.
\end{itemize}

The former is provided to us by the range space of the Hessian. 
The latter can be
obtained by whitening the parameter space. Since the Hessian can vary in
parameter space, another concern will be globalizing the low-dimensional
subspace. 

\begin{remark}
    At this stage it's unclear which Hessian must be used. There are two
    possible candidates - the Hessian of the misfit function, 
    $\nabla^2_{\uq}\left(\frac{1}{2\sigma^2}\left(y - f(\uq)\right)^2\right)$, 
    and the Hessian of
    the parameter-to-QOI map, $\nabla^2_{\uq}f(\uq)$. This is something that
    needs further investigation.
\end{remark}

A very similar dimension reduction problem has been studied in the context of
Bayesian inverse problems~\cite{spantini2015optimal}. In the next subsection,
this strategy is reproduced.

\subsection{Likelihood informed subspaces}

Likelihood informed dimension reduction outlines a strategy to identify a
low-dimensional subspace which captures the change from the prior to the
posterior.
Such a low-dimensional subpsace is expected to exist, since the data aren't
typically informative of all directions in parmaeter space and priors are
typically smoothing. This implies that the likelihood function $p(y | \uq)$
should depend only on a limited number of directions in parameter space. 
If $P_r$ is a rank $r$ projector (i.e., $P_r^2 = P_r$) onto the subpsace that corresponds
to these directions, then, $p(y | P_r\uq)$ should be a good approximation to
$p(y | x)$, since $P_r$ picks out directions to which $p(y | \uq)$ is most
sensitive. These can also be thought of as the directions which are the most
informed by the data. In~\cite{spantini2015optimal}, it is shown that the optimal
projector for affine-Gaussian inverse problems can be constructed as:

\begin{theorem}[Local LIS] 
    Let ${\Sigma}_0 = {L}{L}^T$ be a symmetric
    decomposition of the prior covariance and let $(\lambda_{i}, \vect{v}_i)$ be the
    eigenvalue-eigenvector pairs of the prior-preconditioned Hessian
    $({L}^T {H}{L}$ such that $\lambda_{i} \ge \lambda_{i +
    1}$. Define the directions $\vect{v}_i = {L}\vect{v}_i$ and
    $\vect{w}_i = {L}^{-T}\vect{v}_i$ together with the matrices
    ${U}_r = [\vect{u}_1, \ldots, \vect{u}_r]$ and ${W}_r =
    [\vect{w_1}, \ldots, \vect{w}_2]$. Then the projector on to the local LIS is
    given by ${P}_r = {U}_r {W}_r^T$
\end{theorem}

This idea has been extended to nonlinear $f$ by globalizing the
likelihood-informed subspace. For a globalized subspace, one considers the
dominant eigenspaces of \emph{expected}
prior-preconditioned Gauss-Newton Hessian ${S}$:

\begin{align*}
    {S} = \int_{\mathbb{R}^m} {L}^T
    {H}(\uq){L}p(\uq | y) \mathrm{d}\uq
\end{align*}

The matrix ${S}$ can be estimate via a Monte Carlo approximation. 

\begin{align*}
    \hat{{S}} = \frac{1}{n}\sum_{k = 1}^n
    {L}^T{H(\uq_i)}{L},\quad \uq_k \sim p(\uq | y)
\end{align*}

Let ${V}^{(k)}_r{D}^{(k)}_r{V^{(k)}_r}^T$ be the 
eigendecomposition of ${L}^T{H}(\uq_k){L}$. To construct
the global LIS, consider the eigendecomposition of the Monte Carlo estimator of
the expected Hessian, $\hat{{S}}$, which takes the form:

\begin{align*}
    \left(\frac{1}{n}\sum_{k = 1}^n
        {V}^{(k)}_r{D}^{(k)}_r{V^{(k)}_r}^T
\right)\vect{\psi}_j = \gamma_j\vect{\psi}_j
\end{align*}

Then the global LIS has the non-orthogonal basis ${\Phi}_r =
{L}{\Psi}_r$, where ${\Psi}_r$ contains the $r$
leading eigenvectors, ${\Phi}_r = [\vect{\psi}_1, \ldots,
\vect{\psi}_r]$.

The projector onto the global LIS, ${P}_r$ can be defined as follows:

\begin{definition}[Global LIS projector]
    The projector onto the global LIS is defined as follows.
    \begin{enumerate}
        \item Suppose the LIS basis computed is ${\Phi}_r =
            {L}{\Psi}_r$, where ${\Psi}_r$ 
            is orthonormal.
            Define the matrix ${\Xi}_r =
            {L}^{-T}{\Psi}_r$ such that
            ${\Xi}_r{\Phi}_r = {I}_r$. 
            The projector
            ${P}_r$ has the form ${P}_r = {\Phi}_r
            {\Xi}_r^T$.
        \item Choose ${\Psi}_{\perp}$ so that $[{\Phi}_r,
            {\Phi}_{\perp}]$ forms a complete orthonormal system in
            $\mathbb{R}^n$. Then, the projector ${I} - {P}_r$
            can be written as ${I} - {P}_r =
            {\Phi}_{\perp} \boldsymbol{\Xi}_{\perp}^T$,
            where $\Phi_{\perp} = {L}{\Psi}_{\perp}$ and
            ${\Xi}_{\perp} =
            {L}^{-T}{\Psi}_{\perp}$

        \item This projector enables the decomposition of the parameter 
               space as follows:
        
                \begin{align*}
                    \uq &= {P}_r\uq + ({I} - {P}_r)\uq\\
                        &= {\Phi}_r {\Xi}_r^T\uq +
                    {\Phi}_{\perp}\Xi_{\perp}\uq\\
                        &= \Phi_r\uq_r + \Phi_{\perp}\uq_{\perp}
                \end{align*}
            \end{enumerate}
\end{definition}

As mentioned earlier, the projector $P_r$ picks out the most data-informed
directions. Then, 
an approximate posterior is obtained by writing $\tilde{p}(\uq | y) \approx p(y |
P_r\uq) p(\uq)$. But $\Phi_r$ also diagonalizes $\Sigma_0$ so that $p(\uq) =
p_r(\uq_r) p_{\perp}(\uq_{\perp})$. Hence, the approximate posterior is

\begin{align}
    \label{eq:posterior_decomp}
    \tilde{p}(\uq | y) = p(y | P_r\uq) p_r(\uq_r)p_{\perp}(\uq_{\perp}).
\end{align} 

Knowing
that the posterior is simply $p(\uq)$ in $\text{Range}(\Phi_{\perp})$ precludes
its exploration. This means that the posterior only needs to be explored in
$\text{Range}(\Phi_r)$. 

\subsection{Application to BIMC}

Assuming that the parameter-to-QOI map $f(\uq)$ is smoothing, a factorization
similar to \cref{eq:posterior_decomp} is expected to exist for the ideal IS
density $q^*$ also. That is,

\begin{align}
    \label{eq:ideal_is_decomp_alt}
    \tilde{q}^*(\uq) = \ind_{\DT}(f(P_r\uq))p_{\perp}(\uq_{\perp})p_r(\uq_r)
\end{align}

In this section, we assume that such a projector is known and describe how the
rare event probability computation can benefit. Strategies for constructing this
projector are described in the next section.

One way to proceed is to work only with the approximate ideal distribution in
the low dimensional subspace, $\tilde{q}^*(\uq_r)$. That is, one uses the BIMC
methodology with $f(\Phi_r\uq_r)$ and $p_r(\uq_r)$ to come up with an IS
density, say, $q_r(\uq_r)$. Then, 

\begin{align}
    \begin{split}
    \tilde{\mu} &= \int \ind_{\DT}(f(\Phi_r\uq_r)p_r(\uq_r) \mathrm{d}\uq_r\\
                &= \int \ind_{\DT}(f(\Phi_r\uq_r)\frac{p_r(\uq_r)}{q_r(\uq_r)}
        q(\uq_r)\mathrm{d}\uq_r
    \end{split}
\end{align}


Since for nonlinear $f$, the decomposition \cref{eq:ideal_is_decomp_2} is
approximate, this estimate is expected to have a bias. However, the variance in
$\tilde{\mu}$ is expected to be small. To get rid of the bias, one can construct
an IS distribution in the full parameter space as: $q(\uq) = q(\uq_r)
p_{\perp}(\uq_{\perp})$. Then the probability calculation proceeds as:

\begin{align}
    \begin{split}
    {\mu} &= \int \ind_{\DT}(f(\uq)p(\uq) \mathrm{d}\uq\\
          &= \int
        \ind_{\DT}(f(\uq))\frac{p(\uq)}{q_r(\uq_r)p_{\perp}(\uq_{\perp})}
            q(\uq_r)p_{\perp}(\uq_{\perp})\mathrm{d}\uq_r
    \end{split}
\end{align}


Since BIMC is employed on $r$ dimensional functions and probability
distributions, it is expected to be more accurate, and require lesser storage
requirements. 

\begin{theorem}[Rao-Blackwellisation]\label{thm:bimc_rao_blackwell}
    If $f$ is independent of $\uq_{\perp}$, then no IS distribution $q(\uq_r,
    \uq_{\perp})$ can perform better than its marginal $q_r(\uq_r)$. The two
    distributions will perform equally well iff $q(\uq_r, \uq_{\perp}) =
    q_r(\uq_r)p_{\perp}(\uq_{\perp})$.
\end{theorem}
\begin{proof}

    We begin the proof by defining the importance sampling estimator based on
    $q(\uq_r, \uq_{\perp})$:

    \begin{align}
        \psi(\uq_r, \uq_{\perp}) =
        \frac{\ind_{\DT}(f(\uq_r))p_r(\uq_r)p_{\perp}(\uq_{\perp})}{q(\uq_r, \uq_{\perp})}
    \end{align}

    The Rao-Blackwellized version of this estimator is its conditional
    expectation given $\uq_r$:

    \begin{align}
        \psi_{\mathrm{RB}}(\uq_r) &= \int \psi(\uq_r, \uq_{\perp})
                                    q_{\perp}(\uq_{\perp}, \uq_r)\mathrm{d}\uq_{\perp}\\
                                  &= \int\int
                                     \frac{\ind_{\DT}(f(\uq_r))p_r(\uq_r)p_{\perp}(\uq_{\perp})}{q(\uq_r, \uq_{\perp})}
                                     q_{\perp}(\uq_{\perp} | \uq_r)\mathrm{d}\uq_r\mathrm{d}\uq_{\perp}\\
                                  &= \frac{\ind_{\DT}(f(\uq_r)p_r(\uq_r)}{q_r(\uq_r)}
    \end{align}

    In other words, the Rao-Blackwellized version of $\psi(\uq_r, \uq_{\perp})$
    is nothing but the IS estimator based on the marginal $q_r(\uq_r)$. In
    addition, 

    \begin{align}
        \mathbb{E}_{\uq_r}\left[\psi_{\mathrm{RB}}(\uq_r)\right] 
                                                     &= \int \psi_{\mathrm{RB}}(\uq_r) q_r(\uq_r)\mathrm{d}\uq_r\\
                                                     &= \int \int \psi(\uq_r, \uq_{\perp}) 
                                                        q_{\perp}(\uq_r, \uq_{\perp})q_r(\uq_r)
                                                        \mathrm{d}\uq_r\mathrm{d}\uq_{\perp}\\
                                                     &= \mu
    \end{align}

    Hence, $\psi_{\mathrm{RB}}$ is an unbiased estimator of $\mu$.

    Then, using the relationship between the variance of conditional and unconditional
    expectations, we have,

    \begin{align}
        \mathbb{V}_{\uq_r, \uq_{\perp}}(\psi(\uq_r, \uq_{\perp})) &=
        \mathbb{V}_{\uq_r}\left[\mathbb{E}_{\uq_{\perp} | \uq_r}(\psi(\uq_r, \uq_{\perp}) )\right]
        + \mathbb{E}_{\uq_r}\left[\mathbb{V}_{\uq_{\perp} | \uq_r}(\psi(\uq_r,
        \uq_{\perp}))\right]\\
        &= \mathbb{V}_{\uq_r}\left[\psi_{\mathrm{RB}}\right]
           + \mathbb{E}_{\uq_r}\left[\mathbb{V}_{\uq_{\perp} | \uq_r}(\psi(\uq_r, \uq_{\perp}))\right]
    \end{align}

    Since $\mathbb{V}_{\uq_r, \uq_{\perp}}(\cdot) \ge 0$, the variance of the
    IS estimator based on $q(\uq_r, \uq_{\perp})$ is never smaller than the
    variance of the IS estimator based on $q_r(\uq_r)$. 
    
    The two estimators are
    of equal quality iff $\mathbb{V}_{\uq_{\perp} | \uq_r}\left[\psi(\uq_r,
    \uq_{\perp})\right] = 0$. The variance of a random variable is zero iff it's
    a constant. This implies that $\psi(\uq_r, \uq_{\perp})$ must be independent
    of $\uq_{\perp}$. In other words, $\psi(\uq_r, \uq_{\perp})$ must be
    constant that depends only on $\uq_r$.

    \begin{align}
        \psi(\uq_r, \uq_{\perp}) &=
        \frac{\ind_{\DT}(f(\uq_r))p_r(\uq_r)p_{\perp}(\uq_{\perp})}{q(\uq_r, \uq_{\perp})}\\
        &=
        \frac{\ind_{\DT}(f(\uq_r))p_r(\uq_r)}{q_r(\uq_r)}\frac{p_{\perp}(\uq_{\perp})}{q_{\perp}(\uq_{\perp} | \uq_r)}
    \end{align}
    
    Hence, $p_{\perp}(\uq_{\perp})/q_{\perp}(\uq_{\perp} | \uq_r)$ must be a
    function of $\uq_r$. Since $q_{\perp}(\uq_{\perp} | \uq_r)$ and
    $p_{\perp}(\uq_{\perp})$ are proper distributions, this function must be 1.
    Therefore, we've showed that the two estimators are of equal quality iff
    $q_{\perp}(\uq_{\perp} | \uq_r) = p_{\perp}(\uq_{\perp})$, and thus
    $q(\uq_r, \uq_{\perp}) = q_r(\uq_r)p_{\perp}(\uq_{\perp})$.
\end{proof}
\subsection{Constructing a global projector}

In this subsection, we describe a very rudimentary scheme to construct the
projector $P_r$ for BIMC. 

First, compute the pseudo-MAP point, $\uqmap$ and construct a local
LIS there. Let this initial basis be $\Phi_r^{(1)}$ and its left inverse
be $\Xi_r^{(1)}$. Initialize the sample set $\chi = \{\uqmap\}$. Then,
for $i \ge 1$, enrich the global LIS as follows:

\begin{enumerate}

    \item Proceed with BIMC procedure, but perform all computations in the $r$
        dimensional subspace $\text{Range}({\Xi_r^{(k + 1)}}^T)$. This means minimizing the
        following cost functional to arrive at a new component center instead of
        \Cref{modifiedAugmentedLagrangian}
        \begin{align}
            \mathcal{L}(\uq_r) = \mathcal{U}(\uq_r) + \mathcal{P}(\uq_r)
            + \frac{1}{\mu}\left(y - f(\Phi_r^{(k)}\uq_r)\right)^2
            - \lambda \left(y - f(\Phi_r^{(k)}\uq_r)\right)
            \label{reducedSpaceModifiedAL}
        \end{align}

        where $\uq_r = {\Xi_r^{(k)}}^T\uq$.
       
    \item Let $\uq_r^{k + 1}$ be a minimizer of \Cref{reducedSpaceModifiedAL}.
        Transform $\uq_r^{k + 1}$ back to the original parameter space as
        $\Phi_r^{(k)}\uq_r^{k + 1}$ Enrich the sample set $\chi^{(k + 1)} =
        \chi^{(k)}\cup \{\Phi_r^{(k)}\uq_r^{k + 1}\}$. Compute the dominant
        eigenspace of the expected prior-preconditioned Hessian.

        \begin{align}
            \frac{1}{|\xi^{(k + 1)}|}\sum_{\uq_k \in \xi^{(k + 1)}} L^T H(\uq_k)
            L = \Psi_r \Delta_r \Psi_r^T
        \end{align}

        and update $\Phi_r^{(k + 1)} = L \Psi_r, \Xi_r^{(k + 1)} =
        L^{-T}\Psi_r$. 

    \item Stop the adaptive procedure if the distance between the subspace stops
        changing, or the IS mixture stagnates. If not, go back to the first
        step.

\end{enumerate}

\section{Distance metrics}

There exist several distance measures for which the distance between two
Gaussian mixtures has an analytical expression. Using these measures can offer
significant improvement in run times, since the KL divergence will not have to
be approximated via Monte Carlo sampling. These measures are:

\begin{itemize}
    \item $L^2$ divergence
    \item Jensen-Renyi divergence
    \item Cauchy Schwarz divergence
\end{itemize}

\label{section:distance_metrics}

\section{Proposed work}

We will investigate:

\begin{itemize}
    \item which Hessian is the most informative
    \item the analytical properties of the proposed projector, if
        any
    \item if sampling in the low-dimensional subspace lead to more accurate
        estimates of the rare-event probability?
    \item whether the benefits accrued by sampling in this low-dimensional
        subspace outweight the cost of constructint the LIS. 
    \item the efficacy of the analytical distance measures.
\end{itemize}

\subsection{Contributions}

\begin{itemize}
    \item Hopefully, a rigorous definition of intrinsic dimensionality of the
        posed UQ problem
     \item Working in this low-dimensional subspaces can reduce storage
        requirements for our algorithm.
    \item It also reduces the number of parameters that must be estimated by
        MPMC. 
\end{itemize}

\subsection{Limitations}

\begin{itemize}
    \item Constructing the LIS might prove to be very expensive.  
    \item The dimension reduction procedure might still yield a high-dimensional
        problem.
\end{itemize}

